Relating depth graded and block graded motivic Lie algebras

Using the block filtration as a realisation of the coradical filtration, we study the discrepancy between the depth filtration and the coradical filtration for motivic multiple zeta values. We construct an explicit dictionary between a certain subspace of block graded multiple zeta values and totally odd multiple zeta values and show that all expected relations in the depth graded motivic Lie algebra may be realised in the block graded Lie algebra as the kernel of an explicit map. We also discuss some connections to the uneven Broadhurst-Kreimer conjecture, and outline a possible approach.

==> results.tex <==
\section{Relating the depth and block graded Lie algebras}
The block graded Lie algebra $\mathfrak{bg}$ is canonically isomorphic to the Lie algebra $\mathfrak{rbg}$ generated by the set
\[\{p_{2k+1}(x_1,x_2)=\frac{(1-2^{2k+1})(x_1+x_2)^{2k}-(x_1-x_2)^{2k}}{2^{2k}}\mid k\geq 1\}\]
obtained by taking the standard block-polynomial representation of the block degree 1 part of $\sigma_{2k+1}$ and dividing by $x_1x_2(x_1-x_2)$. It will be convenient to rescale $p_{2k+1}$ so that the coefficient of ``$\zeta(2k+1)$'' is 1. It is equipped with Lie bracket determined for $r(x_1,x_2)$ of block degree 1 and $q(x_1,\ldots,x_{n-1}$ of block degree $n-2$ by the formula
\[\{r,q\}(x_1,\ldots,x_n):=\sum_{i=1}^n r(x_i,x_{i+1})\left(q(x_1,\ldots,\hat{x}_{i+1},\ldots,x_n)-q(x_1,\ldots,\hat{x}_i,\ldots,x_n)\right),\]
where we consider indices modulo $n$ and $\hat{x}_j$ means we omit $x_j$.

Since all polynomials in this Lie algebra are of even total degree, it is easy to check that the projection
\[\pi_e:\bigoplus_{n\geq 2}\mathbb{Q}[x_1,\ldots,x_n]\to \bigoplus_{n\geq 2}\mathbb{Q}[x_1^2,\ldots,x_n^2]\]
onto the part that is even in every variable induces a Lie algebra homomorphism from $\mathfrak{rbg}$ onto its image, which we will denote by $\mathfrak{ebg}$. Denote the image of the generators by $e_{2k+1}(x_1,x_2)$.

From our previous results, we know that $\mathfrak{ebg}$ is isomorphic in block degree at most 2 to the depth graded Lie algebra $\mathfrak{dg}$ in depth at most 2. We claim that we have a surjective partial map $\mathfrak{dg}\to\mathfrak{ebg}$. Specifically, denote by $\mathfrak{sdg}\subset\mathfrak{dg}$ the Lie subalgebra generated by (the depth graded images of) $\{\sigma_{2k+1}\mid k\geq 1\}$. Using the standard stuffle embedding, this can be identified with a Lie subalgebra of $\bigoplus_{n\geq 1}\mathbb{Q}[y_0,\ldots,y_n]$, where the image of $\sigma_{2k+1}$ is $s_{2k+1}(y_0,y_1)=(y_0-y_1)^{2k}$. The Lie bracket of $f(y_0,\ldots,y_r)$ and $g(y_0,\ldots,y_s)$ is given by the antisymmetrization of

\begin{align*}
(f\circ g)(y_0,\ldots,y_{r+s} &{}= \sum_{i=0}^s f(y_i,\ldots,y_{i+r})g(y_0,\ldots,y_i,y_{i+r+1},\ldots,y_{r+s})\\
+(-1)^{\deg f + r}&{}\sum_{i=1}^s f(y_{i+r},\ldots,y_i)g(y_0,\ldots,y_{i-1},y_{i+r},\ldots,y_{r+s})
\end{align*}

Brown \cite{Anatomy of an associator} shows that elements of $\mathfrak{dg}$ satisfy certain dihedral symmetries. In particular, we have that
\[f(y_0,\ldots,y_r) = (-1)^{r+1}f(y_r,\ldots,y_0)\]
and
\[f(y_0,\ldots,y_r)=f(y_1,\ldots,y_r,y_0)\]
for any $f\in\mathfrak{dg}$. Using this dihedral symmetry, we find that the Lie bracket of $f(y_0,y_1)$ and $g(y_0,\ldots,y_{n-2})$ is given by
\[\{f,g\}(y_0,\ldots,y_{n-1})=\sum_{i=0}^{n-1} f(y_i,y_i+1)\left(g(y_0,\ldots,\hat{y}_{i+1},\ldots,y_{n-1})-g(y_0,\ldots,\hat{y}_i,\ldots,y_{n-1})\right).\]
Note that this is identical in form to the Lie bracket for $\mathfrak{bg}$. Furthermore, note that the composition of $y_i\mapsto x_{i+1}$ and $\pi_e$ takes $2s_{2k+1}(y_0,y_1)$ to $(-1)^ke_{2k+1}(x_1,x_2)$. Thus we have a Lie algebra homomorphism
\[\mathfrak{sdg}\to\mathfrak{ebg}\]
that is surjective on the generators, and hence surjective as a morphism of Lie algebras. This extends to a surjection 
\[\mathfrak{dg}\to\mathfrak{ebg}\]
by choosing a set of exceptional generators for $\mathfrak{dg}$ and defining their image to be zero. Thus we have the following.

\begin{theorem}
Via the standard identification with polynomial algebras, projection onto the totally even part defines surjective maps
\begin{align*}
    \mathfrak{bg} &\twoheadrightarrow \mathfrak{ebg},\\
    \mathfrak{sdg} &\twoheadrightarrow \mathfrak{ebg},
\end{align*}
such that the following diagram commutes.
\[\begin{tikzcd}
{} & \Lie [\sigma_3,\sigma_5,\ldots]\arrow[d] \arrow{r}{\simeq} & \mathfrak{bg}\arrow[d]\\
\mathfrak{dg}\arrow[r] & \mathfrak{sdg}\arrow[r] & \mathfrak{ebg}\\
\end{tikzcd}\]
\end{theorem}

I also make the following conjecture. It holds in Lie degree 1 and 2, and holds in Lie degree 3 up to weight 33.

\begin{conjecture}
The map $\mathfrak{sdg}\to\mathfrak{ebg}$ is an isomorphism.
\end{conjecture}

This should be equivalent-ish to the following conjecture:

\begin{conjecture}
    Modulo products, the vector space $\mathcal{D}_n/\left(\mathcal{D}_n\cap\mathcal{B}_{n-1}\right)$ is spanned by totally odd zeta values of depth $n$.
\end{conjecture}

This is the basically the space of elements whose depth is equal to their $f$-degree. This should be equivalent-ish to the uneven Broadhurst-Kreimer conjecture.

A neat corollary to the theorem uses the following, poorly expressed, result.
\begin{theorem}\label{thm:blocktodepthreduction}
    Denote by $\mathcal{E}_{n}$ the vector space of linear functionals on $\mathbb{Q}[x_1,\ldots,x_n]$ spanned by $[x_1^{2m_1}\ldots x_n^{2m_n}]^\vee$ for $m_i\geq 0$, restricted to $\mathfrak{rbg}$. We may view $\I^\mathfrak{l}(\ell_1,\ldots,\ell_r)$ as linear functionals on $\mathfrak{rbg}$ by
    \[\langle \I^\mathfrak{l}(\ell_1,\ldots,\ell_r),-\rangle := \left([x_1^{\ell_1-2}x_2^{\ell_2-1}\ldots x_r^{\ell_r-1}]^\vee - [x_1^{\ell_1-1}\ldots x_{r-1}^{\ell_{r-1}-1}x_r^{\ell_r-2}]^\vee\right).\]

    Similarly, $\zeta_{k_1}^\mathfrak{l}(k_2,\ldots,k_{r})$ defines a linear functional on $\mathfrak{sbg}$ (and hence its image in $\bigoplus_{n\geq 2}\mathbb{Q}[x_1,\ldots,x_r]$) by
    \[\langle \zeta_{k_1}^\mathfrak{l}(k_2,\ldots,k_r),-\rangle := [x_1^{k_1-1},\ldots,x_r^{k_r-1}]^\vee.\]
    Suppose a linear combination $\xi_B$ of block degree $r-1$ iterated integrals of weight $N$ defines a linear functional $\mathcal{F}$ in $\mathcal{E}_{r}$, and a linear combination $\xi_D$ of depth $r-1$ MZVs defines the same linear functional in $\mathcal{E}_r$. Then $\xi_B-2^{r-1}\xi_D=0$ modulo products and terms of lower $f$-degree/block degree.
\end{theorem}

\begin{proof}
    A linear combination $\xi$ of motivic multiple zeta values vanishes modulo products if and only if $\langle \xi,\sigma\rangle=0$ for every $\sigma\in\mathfrak{g}^\mathfrak{m}$. Note that, from standard results about the Ihara bracket, and a result from my thesis, the Lie degree of an element $\sigma$ gives a lower bound on both depth and block degree. That is to say that, for an element $\sigma$ of Lie-degree $m$,
    \[\langle zxi, \sigma\rangle = 0\]
    for all $\xi$ of depth or block degree less than $m$.

    Now suppose $\xi_B$ and $\xi_D$ are as above, of block degree and depth $r-1$ respectively. Then
    \[\langle \xi_B-2^{r-1}\xi_D,\sigma\rangle = 0\]
    for all $\sigma$ of Lie degree at least $r$. Suppose $\sigma$ is of Lie degree exactly $r-1$ and is given by some Lie polynomial
    \[\sigma = P(\sigma_3,\sigma_5,\ldots,\sigma_{2N+1})\]
    Since the block degree $r-1$ part of $\sigma$ is given by the same Lie polynomial applied to the block degree 1 parts of $\sigma_{2k+1}$, we must have that
    \[\langle \xi_B,\sigma\rangle = \langle \xi_B, P(p_3,\ldots,p_{2N+1})\rangle\]
    However, by assumption, $\xi_B$ defines a totally even functional. Thus
    \[\langle \xi_B,\sigma\rangle = \langle \xi_B, \pi_eP(p_3,\ldots,p_{2N+1})\rangle = \langle\xi_B, P(e_3,\ldots,e_{2N+1})\rangle.\]
    Similarly, we must have that
    \[\langle \xi_D,\sigma\rangle = \langle \xi_D, \pi_e P(s_3,\ldots,s_{2N+1})\rangle = \langle 2^{r-1}\xi_D, P(e_3,\ldots,e_{2N+1})\rangle.\]
    Since $P(e_3,\ldots,e_{2N+1})$ is totally even
    \[\langle \xi_B,P(e_3,\ldots,e_{2N+1}\rangle = \mathcal{F}(P(e_3,\ldots,e_{2N+1}))=\langle 2^{r-1}\xi_D,P(e_3,\ldots,e_{2N+1})\rangle\]
    and so $\langle \xi_B-2^{r-1}\xi_D,\sigma\rangle=0$ for all $\sigma$ of Lie degree $r-1$. 
    If $\langle \xi_B-2^{r-1}\xi_D,\sigma\rangle\neq 0$ for $\sigma$ of Lie degree less than $r-1$, we can always add terms of lower Lie/$f$ degree to cancel out the contribution without affecting higher Lie degree. Thus, up to addition of terms of lower degree $\xi_B-2^{n-1}\xi_D$ annihilates all of $\mathfrak{g}^\mathfrak{m}$, and hence the result holds.
\end{proof}

Surjectivity of the map $\mathfrak{sdg}\to\mathfrak{ebg}$ tells us that, given such a $\xi_B$, we can always construct the corresponding $\xi_D$.
\begin{corollary}
If $\xi_B$, of block degree $n$ defines a totally even functional, $\xi_B$ can be (explicitly) expressed in terms of totally odd multiple zeta values of depth $n$, modulo products and terms of lower block degree.
\end{corollary}

\begin{corollary}
    Up to some rational factor
    \[\sum_{i=a}^{n-a}\zeta^\mathfrak{l}(\{2\}^i,6,\{2\}^{n-i})=-16\zeta^{\mathfrak{l}}(1,1,2n-2a+1,2a+3)\]
    modulo products and block degree $3$.
\end{corollary}
\begin{proof}
    It is easy to check that the left hand side defines, up to a rational factor, the functional $-[x_1^{2a+2}x_5^{2n-2a}]^\vee$, which, via the cyclic symmetry, defines the same linear functional on $\mathfrak{rbg}_4$ as $-[x_4^{2n-2a}x_5^{2a+2}]^\vee$. This is the same linear functional defined by $-\zeta^\mathfrak{l}(1,1,2n-2a+1,2a+3)$. Hence, modulo products and terms of lower block degree,
    \[\sum_{i=a}^{n-a}\zeta^\mathfrak{l}(\{2\}^i,6,\{2\}^{n-i})=-16\zeta^{\mathfrak{l}}(1,1,2n-2a+1,2a+3)\]
\end{proof}

Numerical evidence suggests that \autoref{thm:blocktodepthreduction} can be strengthened to a result that holds not just modulo terms of lower block degree, but modulo terms of lower depth. This seems to be closely related to both Brown's uneveness conjecture, and the homological Broadhurst Kreimer conjecture.

\begin{conjecture}
    Relations coming from the above theorem hold modulo terms of lower depth. That is to say that $\langle \xi_B-2^{r-1}\xi_D,\sigma\rangle=0$ for any elements in the Lie ideal generated by the exceptional generators in $\mathfrak{dg}$ of depth $r-1$. 
\end{conjecture}
\todo[inline]{Check the sign of the factor of 2}

\begin{lemma}
    The map $\mathfrak{sdg}\to\mathfrak{ebg}$ is an isomorphism?
\end{lemma}
\begin{proof}
    We know that this map defines a surjection, and so it suffices to show that it is an injection, i.e. if $f(y_0,\ldots,y_n)\in\mathfrak{sdg}$ has zero totally even part, then $f$ is zero. Since projection onto the totally even part commutes with setting $y_0$ to $0$, and $f$ is translation invariant, we it suffices to show this claim holds for 
    \[\bar{f}(y_1,\ldots,y_n):=f(0,y_1,\ldots,y_n).\]
    Since $\mathfrak{sdg}$ is a subspace of the depth graded motivic Lie algebra, and hence a subspace of the Lie algebra associated to the linearised double shuffle equations. The shuffle equation tells us that, for any non trivial shuffle of $y_1,\ldots,y_n$, the corresponding sum of
    \[\bar{f}(y_1,y_1+y_2,y_1+y_2+y_3,\ldots,y_1+\cdots+y_n)\]
    vanishes. For notational convenience, from here we omit the bar over $f$. We may write the above polynomial as
    \[e^{y_1\frac{\partial}{\partial y_2}}e^{y_2\frac{\partial}{\partial y_3}}\cdots e^{y_{n-1}\frac{\partial}{\partial y_n}}f(y_1,\ldots,y_n).\]
    Denoting by $D_{i,j}:=y_i\frac{\partial}{\partial y_j}$, we can thus rewrite the $(p,q)$-shuffle equation as
    \[\sum_{\sigma\in\mathcal{S}_{p,q}} \left(\prod_{i=1}^{n-1}e^{D_{\sigma(i),\sigma(i+1)}}\right)f(y_{\sigma(1)},y_{\sigma(2)},\ldots,y_{\sigma(n)}=0\]
    where the product of differential operators is ordered. I have no idea where to go from here, but it seems like an approach?
\end{proof}

\begin{remark}
        The linearised stuffle equations tell us that, for example
    \[f(y_1,\ldots,y_n)+\sum_{i=2}^n f(y_2,\ldots,y_i,y_1,y_{i+1},\ldots,y_n)=0\]
    and this clearly restricts to the totally even part and hence to the image of $y$ in $\mathfrak{ebg}$ (i.e. it's even part up to a power of $2$. Thus, the following holds in $\mathfrak{ebg}$
    \[f(0,x_2,\ldots,x_{n+1}+\sum_{i=3}^{n+1}f(0,x_3,\ldots,x_{i},x_{2},x_{i+1},\ldots,x_{n+1}) = 0.\]
    To compare, the block shuffle relation tells us that
    \[f(x_1,x_2,\ldots,x_{n+1}+\sum_{i=3}^{n+1}f(x_1,x_3,\ldots,x_{i},x_{2},x_{i+1},\ldots,x_{n+1}) = 0.\]
    Thus, this case of the linearised stuffle equation could be viewed as a reflection of this very special case of the block shuffle relation.

    In general, block shuffle says that the sum over shuffles of $(x_1-x_n)f(x_1,\ldots,x_n)$ vanishes for $f\in\mathfrak{rbg}$, and I don't think it is possible to rephrase this without the pre-factor in general. However, in up to 6 variables, it is always possible to rewrite the block shuffle relations purely in terms of $\mathfrak{rbg}$ - in fact, all block shuffle relations in up to six variables follow from the above relation and the dihedral symmetries. This seems to break down for 7 variables - the dihedral symmetry gets too weak there.
\end{remark}



